ELSA: Efficient Long-Term Secure Storage of Large Datasets

An increasing amount of information today is generated, exchanged, and stored digitally. This also includes long-lived and highly sensitive information (e.g., electronic health records, governmental documents) whose integrity and confidentiality must be protected over decades or even centuries. While there is a vast amount of cryptography-based data protection schemes, only few are designed for long-term protection. Recently, Braun et al. (AsiaCCS'17) proposed the first long-term protection scheme that provides renewable integrity protection and information-theoretic confidentiality protection. However, computation and storage costs of their scheme increase significantly with the number of stored data items. As a result, their scheme appears suitable only for protecting databases with a small number of relatively large data items, but unsuitable for databases that hold a large number of relatively small data items (e.g., medical record databases). In this work, we present a solution for efficient long-term integrity and confidentiality protection of large datasets consisting of relatively small data items. First, we construct a renewable vector commitment scheme that is information-theoretically hiding under selective decommitment. We then combine this scheme with renewable timestamps and information-theoretically secure secret sharing. The resulting solution requires only a single timestamp for protecting a dataset while the state of the art requires a number of timestamps linear in the number of data items. We implemented our solution and measured its performance in a scenario where 12 000 data items are aggregated, stored, protected, and verified over a time span of 100 years. Our measurements show that our new solution completes this evaluation scenario an order of magnitude faster than the state of the art.

==> include/addfunc.tex <==
%!TEX root = efficient_lincos.tex

\section{Additional Functionalities}
\label{sec.addfunc}

\subsection{Format Migration}
\todo{revise this section. maybe exclude?}
\Lincomo{} is supposed to protect data for decades or even centuries.
During such a long time period new data formats are developed and deployed.
For the stored data to remain useful it is desirable that the storage system supports a procedure for secure format migration.
It should be possible to migrate the data format without losing integrity protection.

%A challenge of format migration in our secure storage architecture is to preserve integrity protection during the migration process.
%For example, if the data is migrated to format Office 2020, it must be ensured that the semantics of the data did not change compared to the semantics of the originally signed data object in format Office 2010.

Data format migration for \Lincomo{} can be realized using an idea proposed by Haber and Kamat \cite{Haber:2006:2161-8798:159}.
Suppose a data object $\dat$ of some old format needs to be migrated to a new format.
The idea is to use a transformation function $F$ that transforms the data to the new format and at the same time is certified to not change the semantics of the data object.
The certified transformation function $F$ is then attested together with the old and the new data object so that the validity of the transformation can be verified.

The above approach for secure format transformation seems to work well for the timestamp-based integrity system.
For the notary-based integrity system, however, one would need to prove to the notarial authority in zero knowledge that the new commitment opens to a transformation of the document to which the old commitment opens to.
We leave the realization of such a zero knowledge proof as an interesting open problem for future work.


\subsection{Commitment Renewal Without Data Owner}

Our long-term secure storage architecture \Lincomo{} uses unconditionally hiding commitments to not leak information about the protected data to attestation services.
These commitments are only computationally binding and need to be renewed from time to time.
Commitment renewal requires the data owner to retrieve the secret data from the storage servers and create a new commitment.
It would be desirable to have a system that renews the protection autonomously, i.e., without the help of the data owner.
%does not require the data owner to become active in order to renew the protection.

In the following we discuss two approaches for autonomous commitment renewal by the storage servers.
The proposed solutions are compatible with sequence-based data structures.
We leave the development of similar solutions for attestation-based data structures for future work.

\subsubsection{Commitment to Share.}
The idea of this approach is that for commitment renewal each storage server $i$ creates a commitment $(c_i,d_i) \gets \Com(s_i)$ to its current share $s_i$.
Then it adds commitment value $c_i$ to the integrity proof at the evidence service, creates a secret sharing $s'_1,\ldots,s'_n$ of its share and the new decommitment value $(s_i,d_i)$, and distributes the shares $s'_1,\ldots,s'_n$ to the storage servers.
At verification of such an integrity proof, the integrity of the sharing at this point can be verified by opening the commitments produced by the storage servers.

%This works as follows.
%Suppose data object $\dat$ was committed to by a commitment $(c,d)$ and secret $s=(\dat,d)$ is shared among a set of storage servers $S_1,\ldots,S_n$, where $S_i$ holds share $s_i$.
%The commitment renewal of $(c,d)$ works as follows.
%
%\begin{enumerate}
%\item
%Every storage server $S_i$ computes a new commitment $(c_i',d_i')$ to its current share $s_i$.
%\item
%Storage server $S_i$ creates a secret sharing $s^{d'}_{i,1},\ldots,s^{d'}_{i,n}$ of $(s_i,d'_i)$ and sends share $s^{d'}_{i,j}$ to storage server $S_j$.
%\item
%Storage server $S_i$ sends commitment value $c_i'$ to the integrity system. Once the integrity system obtained $(c_1',\ldots,c_n')$, it requests a new attestation for $(c_1',\ldots,c_n')$.
%\end{enumerate}
%
%Verification of such a distributed commitment works as follows.
%For each share $s_i$, the validity of the corresponding commitment $(c_i',d_i')$ is checked. Additionally, it is checked that the attestation sequence guarantees that the commitments $(c_1',\ldots,c_n')$ were made when the previous commitment was still valid.

The above approach for commitment update without the data owner does not require the invention of new cryptographic techniques.
However, its performance decreases over time as the size of the stored data increases significantly with each commitment update.

\subsubsection{Recommitment via Multiparty Computation.}

Another approach for autonomous commitment updates by the storage servers is to use secure multiparty computation.
The idea is that the storage servers run a secure multi party computation protocol that computes a new commitment to the stored data similar to Algorithm~\ref{alg.update}.
It is known that any function on inputs of the storage servers can be computed without compromising the confidentiality of the input data \cite{DBLP:conf/stoc/GoldreichMW87}.
However, the general protocol constructions are not efficient in practice.
Realizing this approach would require developing a specifically tailored secure multiparty computation protocol for creating a commitment without revealing the committed data.
%
%Suppose a data object $\dat$ was commited to by a commitment $(c_1,d_1)$, attested by attestation $a_1$, and secret $s=(\dat,d_1)$ is shared among a set of storage servers $S_1,\ldots,S_n$, where $S_i$ holds share $s_i$.
%We consider a secure multiparty computation protocol $P$ that on input of shares $s_1,\ldots,s_n$, computes a commitment $(c_2,d_2)$ to $(\dat,d_1)$. After the protocol has finished each storage server $S_i$ obtained the commitment value $c_2$ in plaintext and a secret share $s^{d_2}_i$ of the decommitment value $d_2$.
%%
%The commitment renewal consists of the following steps.
%\begin{enumerate}
%\item
%The storage servers on input of their shares run protocol $P$ and storage server $S_i$ obtains commitment value $c_2$ and decommitment share $s^{d_2}_i$.
%\item
%Each storage server $S_i$ sends the commitment value $c_2$ to the integrity system.
%The integrity system checks whether all the received commitment values are the same and if this is the case, retrieves a new attestation $a_2$ for the commitment $c_2$ and adds it to the attestation sequence.
%\end{enumerate}
%
%The resulting data structures do not differ from the ones described in Section~\ref{sec.modint}, where the data owner renews the commitment.
%Indeed, the storage servers use the protocol $P$ to mimic the recommitment that is done by the data owner in the original solution.
%Hence, the verification of a proof of existence where recommitments are performed using multiparty computation works the same as the verification of a proof of existence where recommitments are performed by the data owner.
%
%Recommitment via multiparty computation is an elegant way to renew commitments without the data owner and without having to change the underlying data structures.
%However, even though it is known that the proposed solution can be realized \cite{DBLP:conf/stoc/GoldreichMW87}, it is unclear how to realize it such that practical performance is achieved.

==> include/conclusions.tex <==
%!TEX root = ../main.tex

\section{Conclusions}
\label{sec.conc}

We have proposed {\ELSA}, a long-term secure storage architecture that provides efficient protection of large data sets.
{\ELSA} drastically improves over the performance of the state of the art when large datasets with small individual items are concerned, as they often occur in practice.
We achieve with {\ELSA} nearly constant computation and storage costs for timestamp renewal by using a new type of vector commitment, while for existing solutions these costs scale linearly with the number of stored items.
Our performance measurements show that \ELSA{} provides practical performance for application scenarios where the stored data consists of many small individual data items, e.g., long-term secure storage of electronic health records.

We envision the following research directions for future work.
It would be interesting to investigate how to combine our vector commitments with ORAM technology in order to obtain a storage architecture that additionally provides long-term access pattern hiding security.
Another interesting direction is to combine secure multiparty computation protocols with our storage architecture in order to allow for computation on the stored and protected data.
Also, it would be interesting to see whether commitment renewal without the help of the data owner is possible.

==> include/confsys.tex <==
%!TEX root = efficient_lincos.tex

\section{Confidentiality System of \Lincomo{}}
\label{sec.modconf}

\todo{Reviewers: each of the confidentiality systems already exist in literature $\to$ no contribution $\to$ either: compress this part and put it somewhere else (e.g., in a different section), or: clearly mention that this is not a main technical contribution but a description and evaluation}
We now present the enhanced confidentiality system of \Lincomo{}.
The confidentiality system allows storage of confidential data at third party storage servers with different protection levels.
%It provides methods $\Store$ for storing data, $\Retrieve$ for retrieving data, and $\Renew$ for renewing the protection.
%We discuss a possible instantiation for each protection level.
%The data owner chooses for each data object which protection level is required.
%For rigorous long-term confidentiality protection, information theoretic security is required as explained in Section~\ref{sec.ltconf}.
%However, achieving information theoretic security is expensive and trade-offs may be desired in certain scenarios.


\subsection{Computational Security}

\subsubsection{Instantiation.}
The computationally secure instantiation of the confidentiality system of \Lincomo{} works as follows.
For protection of data in transit, the private channels are instantiated using a traditional TLS connection, that is, using a computationally secure key exchange protocol (e.g., Diffie-Hellman Key Exchange) and a computationally secure symmetric encryption scheme (e.g., AES).
%
For computationally secure protection of data at rest, a symmetric encryption scheme is chosen (e.g., AES) for encrypting the data and the ciphertexts are stored at a storage server.
Protection renewal is performed by chosing a new encryption scheme and re-encrypting all the stored data.
We stress that this protection renewal does not protect against a malicious storage server or the if the old ciphertexts have already been eavesdropped by an attacker.

%a symmetric encryption scheme is used and only a single storage server for storing the encrypted data. Secret sharing is not applied in this case.
%For storing data, the data owner first encrypts the data to a ciphertext using a symmetric encryption scheme.
%It sends the ciphertext to the storage server and stores the private decryption key locally.

\if{false}
When method $\Store(\dat)$ is called, the data $\dat$ is encrypted to a ciphertext $c$, and $c$ is sent over a private channel to the storage server.
When method $\Retrieve()$ is called, the user retrieves the ciphertext $c$ (after authentication with the storage server), and decrypts $c$ to $\dat$.
If the currently used encryption scheme is expected to become insecure in foreseeable future, method $\Renew()$ can be used to replace the encryption scheme.
When method $\Renew()$ is called, the user retrieves $c$ and decrypts $c$ to $\dat$.
Then, it uses a new encryption scheme to encrypt $\dat$ to $c'$ and sends $c'$ to the storage server.
We stress that this kind of protection renewal does only protect against attackers who might break into the storage server after the renewal. However, it does not help if the storage server itself is malicious. A malicious storage server can store the old ciphertext and run a brute force attack in the future.
\fi

\subsubsection{Properties.}
%Computational security for confidentiality protection is sufficient if the required protection period is short period (e.g., less than five years), the protected data is not highly sensitive, or expensive information theoretically secure protection cannot be afforded.
The computationally secure confidentiality system has low storage requirements and very good performance.
Only a single storage server is required that stores encrypted data of size similar to the original data.
Storage throughput performance is practically only limited by the bandwidth of the network connection between the data owner and the storage server and the performance of the symmetric encryption scheme.
%Hence, the performance of this instantiation of the confidentiality system is most likely sufficient for almost any application scenario.

\subsubsection{Security.}
It is easy to see that the confidentiality system instantiated with computationally secure components protects the confidentiality of the stored data if the adversary has a \emph{fixed} computational bound.
Therefore, it provides sufficient security for a limited period of time (e.g., a few years).
However, the system is not secure against attackers that collect encrypted data (when eavesdropping on network channels or after breaking into a storage server) and then run a brute force attack to break the encryption later.


\subsection{Information-Theoretic Security}
%Information theoretic confidentiality protection is used if the data needs protection over long time periods (e.g., decades or centuries) or is highly sensitive.
%In such a case, the confidentiality system of \Lincomo{} is instantiated with information theoretically secure components.

\subsubsection{Instantiation.}
To provide information theoretic security, the confidentiality system is instantiated similar to the confidentiality system of \Lincos{}.
For data in transit, the private channels are instantiated using QKD \cite{RevModPhys.74.145} and one-time pad encryption \cite{BLTJ:BLTJ928}.
For data at rest, information theoretically secure proactive secret sharing \cite{DBLP:conf/crypto/HerzbergJKY95} in combination with a set of storage servers is used.

\if{false}
When method $\Store(\dat)$ is called, secret shares $s_1,\ldots,s_n$ of the data $\dat$ are computed and sent to the storage servers.
When method $\Retrieve()$ is called, the user retrieves the shares $s_1,\ldots,s_n$ (after authentication with the storage servers), and reconstructs the data $\dat$ from the shares.
When method $\Renew()$ is called, the user runs the share renewal protocol of the proactive secret sharing scheme so that an attacker will not be successful in stealing one share after another over time.
\fi

\subsubsection{Properties.}
The information theoretically secure instantiation of the confidentiality system offers a very high protection, but comes at a significant cost in performance and practicability.
%
Even though QKD is currently the most practical solution for realizing information theoretically secure key exchange, it is not yet widely available and its performance is limited.
%
Moreover, using secret sharing for storing confidential data means that a multiple of the original data size must be sent over the network and stored at the storage servers.

On the positive side, secret sharing schemes allow for robustness against storage server failures because the data is distributed among several storage servers and is recoverable even if some servers fail.
Furthermore, secret sharing allows for managing different access structures to the data, for example, using hierarchical secret sharing \cite{traverso2016}.

\subsubsection{Security.}
It is easy to see that the confidentiality system instantiated with information theoretically secure components is secure against a computationally unbounded adversary who eavesdrops on the private channels and breaks into a small subset of the storage servers.
Remarkably, this instantiation of the confidentiality system is secure against any kind of brute force attack.
Therefore, the protection level is suitable for highly sensitive data that needs to be protected for long time periods (e.g., several decades or even centuries).
We stress that in this case periodic renewal of the shares is important to protect against mobile adversaries that succeed in breaking into several storage servers over time.


\if{false}
\subsection{Hybrid Solutions}
In some scenarios, the protection requirements for data in transit and data at rest may be different and the confidentiality system may be instantiated combining computationally secure components with information theoretically secure components.

%\subsubsection{Comp.\ Sec.\ In-Transit and Inf.\ Theo.\ Sec.\ At-Rest}
Combining computationally secure private channels with information theoretically secure secret sharing may be suitable for situations where information theoretically secure private channels (e.g., using QKD) are not available or too expensive and at the same time high protection and flexible access management at the storage server side must be provided.
Such an instantiation benefits from the high throughput performance of computationally secure channels and the robustness against storage server failures of the secret sharing storage system.
It may be suitable for private users and small companies who cannot afford to use QKD, but still want a flexible, secure, and robust storage solution.

%\subsubsection{Inf.\ Theo.\ Sec.\ In-Transit and Comp.\ Sec.\ At-Rest}
A combination of information theoretically secure private channels and computationally secure storage may be suitable for situations where highly sensitive data is concerned and sent over a public network, but the storage system is controlled by the same entity that owns the data.
The solution benefits from requiring only a small storage server infrastructure consisting of a single storage server.
\fi

%If computationally security is sufficient for data-at-rest but the data sent over the network must be highly protected, information theoretic secure private channels can be combined with computationally secure encryption for protecting the stored data.
%This solution may be relevant for companies that want to send highly sensitive data over a public network to another data center that is also controlled by the company and only needs medium protection against unauthorized access to the data from employees.

%\subsubsection{Hybrid Security}
%In cases where a subset of the nodes in the network are connected via information theoretically secure private channels, but other nodes are only connected via computationally secure private channels, a combination of information theoretic secure private channels and computationally secure private channels is used.
%The idea is to cluster the network such that the communication between the clusters is carried out over information theoretically secure channels, but the communication within the clusters has a lower threat level and is carried out over computationally secure private channels. This approach is described in more detail in \cite{brendel2016}.
%\MG{performance figures showing the speedup achieved through this?}
%
%Furthermore, if information theoretic security can only be provided for a subset of the network channels, a hybrid solution for securing data in transit can be used that efficiently combines information theoretic secure private channels with computationally secure private channels as described in \cite{brendel2016}.

\if{false}
\subsection{Comparison}
In Table~\ref{tab.modconfcompare} we compare the computationally secure confidentiality system with the information theoretically secure confidentiality system.
Here we assume a network connection performance of \SI{1}{\giga\bit\per\second} for computationally secure channels and a QKD key exchange performance of \SI{1}{\mega\bit\per\second}, which reflects the performance of currently available technology \cite{Sasaki:11}.
The table summarizes that while performance is better using computationally secure components, information theoretically secure components provide better security, flexibility, and robustness.
The hybrid solutions share benefits and drawbacks of the computationally and information theoretically secure solutions, respectively.

\begin{table}
\center

\caption{\label{tab.modconfcompare} Comparison of the computationally secure and the information theoretically secure confidentiality system of \Lincomo{} for $n$ storage servers.}

\begin{tabular}{ | l | c | c | }
\hline
& \textbf{Comp.\ Security} & \textbf{Inf.\ Theo.\ Security} \\ \hline\hline

Time (Store \SI{1}{\giga\byte}) &
$\sim$ \SI{8}{\second}
&
$\sim$ \SI{2.2}{\hour}
\\ \hline

Space (Store \SI{1}{\giga\byte}) &
$\sim$ \SI{1}{\giga\byte}
&
$\sim$ $n * \SI{1}{\giga\byte}$
\\ \hline

Long-Term Security &
\xmark
&
\cmark
\\ \hline

Flexible Access Control &
\xmark
&
\cmark
\\ \hline

Robust to Server Failures &
\xmark
&
\cmark
\\ \hline
\end{tabular}

\end{table}
\fi
